Study of $e^+e^-\to \Upsilon(\rm1S,2S)\eta$ and $e^+e^-\to \Upsilon(\rm 1S)\eta^{\prime}$ at $\sqrt{s}=10.866$ GeV with the Belle detector

We report the first observation of the processes $e^+e^-\to\Upsilon(\rm 1S,2S)\eta$ at $\sqrt{s}=10.866$~GeV with a $10.2\sigma$ and $16.5\sigma$ significance respectively. The measured Born cross sections are $\sigma(e^+e^- \to \Upsilon(2S)\eta)=2.07 \pm 0.21 \pm 0.19$~pb, and $\sigma(e^+e^- \to \Upsilon(\rm 1S)\eta)=0.42 \pm 0.08 \pm 0.04$~pb. We also set the upper limit on the cross section of the process $e^+e^- \to \Upsilon(\rm 1S)\eta^{\prime}$ to be $\sigma(e^+e^- \to \Upsilon(\rm 1S)\eta^{\prime})<0.035$~pb at $90\%$ CL. The results are obtained with the data sample collected with the Belle detector at the KEKB asymmetric-energy $e^+e^-$ collider in the energy range from $10.63$~GeV to $11.02$~GeV.

==> biblio.tex <==
\begin{thebibliography}{99}

\bibitem{Kou:2018nap}

\bibitem{Yamada2014}

\bibitem{Agostinelli:2002hh}

\bibitem{Abe:2010gxa}

\bibitem{Belle-ECL:2015vma}

\bibitem{Moll:2011zz}

\bibitem{Calame:2019ysp}

\bibitem{PDG}

\bibitem{GEANT}

\bibitem{root}

\bibitem{FNAL}

\bibitem{CLEO}

\bibitem{Babar}

\bibitem{Voloshin:2011hw}

\bibitem{Voloshin:2012dk}

\bibitem{Aubert:2008az}

\bibitem{BABAR:2011ab}

\bibitem{Voloshin:1980zf}

\bibitem{Guido:2018ywg}

\bibitem{Kurokawa:2001nw}

\bibitem{Abashian:2000cg}

\bibitem{Lange:2001uf}

\bibitem{Voloshin:2006ce}

\bibitem{PHOTOS}

\bibitem{Fadin}

\bibitem{hb_scan}

\bibitem{Ypipi_scan}

\bibitem{Voloshin:2007dx}

\bibitem{eta-prime}

\bibitem{Garmash:2014dhx}

\bibitem{Mizuk:2012pb}

\bibitem{Eichten:2005ga}

\bibitem{Ypipi_scan_new}

\bibitem{Krokovny}

  
\end{thebibliography}


